Safe Risk-averse Bayesian Optimization for Controller Tuning

Controller tuning and parameter optimization are crucial in system design to improve both the controller and underlying system performance. Bayesian optimization has been established as an efficient model-free method for controller tuning and adaptation. Standard methods, however, are not enough for high-precision systems to be robust with respect to unknown input-dependent noise and stable under safety constraints. In this work, we present a novel data-driven approach, RaGoOSE, for safe controller tuning in the presence of heteroscedastic noise, combining safe learning with risk-averse Bayesian optimization. We demonstrate the method for synthetic benchmark and compare its performance to established BO-based tuning methods. We further evaluate RaGoOSE performance on a real precision-motion system utilized in semiconductor industry applications and compare it to the built-in auto-tuning routine.

==> sections/10-list_of_symbols.tex <==

\nomenclature{$\Pkp$}{Position proportional gain}
\nomenclature{$\Vkp$}{Velocity proportional gain}
\nomenclature{$\Vki$}{Velocity integral gain}
\nomenclature[$\Vff$]{Velocity feedforward gain}
\nomenclature[$\Aff$]{Acceleration feedforward gain}
\nomenclature{$\domain$}{Space of admissible controllers}
\nomenclature{$f$}{Objective (Average tracking error)}
\nomenclature{$q_1$}{Safety constraint (FFT of the torque)}
\nomenclature{$q_2$}{Performance constraint (Max tracing error)}
\nomenclature{$\mu$}{GP mean}
\nomenclature{$k$}{GP kernel}
\nomenclature{$\data$}{Data set}
\nomenclature{$\task$}{Task parameter}
\nomenclature{$l_t(x)$}{Lower bound of confidence interval}
\nomenclature{$u_t(x)$}{Upper bound of confidence interval}
\nomenclature{$\X_{0}$}{Initial safe seed}
\nomenclature{$\g{x}{z}$}{Optimistic noisy expansion operator}
\nomenclature{$\X^{opt}_{t}$}{Optimistic safe set}
\nomenclature{$\suggestion$}{Recommendation of PSO}
\nomenclature{$x_w^*$}{Expander}
\nomenclature{$z_i$}{$i^{th}$ particle best position}
\nomenclature{$\overline{z}_i$}{Overall particles best position}
\nomenclature{$\X_t$}{Safe set}
\nomenclature{$L_t$}{Safe set boundary}
\nomenclature{$L_q$}{Lipschitz constant}
\nomenclature{$W_t$}{Uncertain points on safe set boundary}
\nomenclature{$\xbest(\task)$}{Feasible controller corresponding to best observed cost for task $\task$}
\nomenclature{$\xbestgrid(\task)$}{Best feasible controller computed with grid search for task $\task$}

\printnomenclature


==> sections/4-background.tex <==
\section{Background}\label{sec:backgound}
%
% \mypar{Gaussian processes}
% A Gaussian process (GP) \cite{Rasmussen} is a distribution over the space of functions commonly used in non-parametric Bayesian regression. It is fully described by a mean function $\mu:\domain \rightarrow \mathbb{R}$, which, w.l.o.g, we set to zero for all inputs $\mu(x)=0,~\forall x\in \domain$, and a kernel function $k:\domain \times \domain \rightarrow \mathbb{R}$. Given the data set $\data=\{(x_i,y_i\}_{i=1}^t$, where $y_i=f(x_i)+\varepsilon_i$ and $\varepsilon_i\sim \mathcal{N}(0,\sigma^2)$ is zero-mean i.i.d. Gaussian noise, the posterior belief over the function $f$ has the following mean, variance and covariance:
% %
% \begin{align}
%     &\mu_t(x) = \mathbf{k}_t^\top(x) (\mathbf{K}_t + \sigma^2 \mathbf{I})^{-1} \mathbf{y}_t, \label{eq:GPmean}\\
%     &k_t(x,x')=k(x,x') - \mathbf{k}_t^\top(x) (\mathbf{K}_t + \sigma^2 \mathbf{I})^{-1} \mathbf{k}_t(x'), \label{eq:GPcovar}\\
%     &\sigma_t(x)=k_t(x,x)\label{eq:GPvar},
% \end{align}
% %
% where ${\mathbf{k}_t(x)=(k(x_1,x), \dots, k(x_t,x))}$, $\mathbf{K}_t$ is the positive definite f matrix $[k(x,x')]_{x,x' \in \data_t}$, and $\mathbf{I} \in \mathbb{R}^{t \times t}$ denotes the identity matrix. In the following, the superscripts $f$ and $q$ denote GPs on the objective and on the constraints.

\mypar{Multi-task BO}
In multi-task BO, the objective depends on the  extended input $(x,\task) \in \domain \times \tdomain$, where $x$ is the variable we optimize over and $\task$ is a task parameter set by the environment that influences the objective. To cope with this new dimension, multi-task BO uses GPs with kernels of the form $k_\text{multi}((x,\task),(x',\task')) = k_{\task}(\task,\task')\otimes k(x,x')$, where $\otimes$ denotes the Kronecker product. This kernel decouples the correlations in objective values along the input dimensions, captured by $k$, from those across tasks, captured by $k_\task$ \cite{Swersky2013}.

\mypar{\goose{}}
\looseness=-1
% \goose{} extends any standard BO algorithm to provide high-probability safety guarantees in presence of \textit{a priori} unknown safety constraints. It builds a Bayesian model of the constraints from noisy evaluations based on GP regression. It uses this model to build estimates of two sets: the \emph{pessimistic} safe set, which contains inputs that are safe, i.e., satisfy the constraints, with high probability and the \emph{optimistic} safe set that contains inputs that could potentially be safe. At each round, \goose{} communicates the optimistic safe set to the BO algorithm, which returns the input it would evaluate within this set, denoted as $\suggestion$. If $\suggestion$ is also in the pessimistic safe set, \goose{} evaluates the corresponding objective. Otherwise, it evaluates the constraints at a sequence of provably safe inputs, whose choice is based on a heuristic priority function, that allow us to conclude that $\suggestion$ either satisfies or violates the constraints with high probability. In the first case, the corresponding objective value is observed. In the second case, $\suggestion$ is removed from the optimistic safe set and the BO algorithm is queried for a new suggestion. Compared to \cite{sui2018stagewise,Sui}, \goose{} achieves a higher sample efficiency \cite{turchetta2019safe} while compared to \cite{Gardner,hernndezlobato2015predictive,picheny2016bayesian,gramacy2016modeling,ariafar2019admmbo}, it guarantees safety at all times with high probability, under  regularity assumptions.



% To start collecting data safely, \goose{} requires knowledge of a set of inputs that are known \textit{a priori} to be safe, denoted as $S_0$. In our problem, it is easy to identify such set by designing conservative controllers for simplistic first principle models of the system under control.

==> sections/7-experimental_results.tex <==
\section{Experimental results}
\label{sec:experimental}

